GeoReF: Geometric Alignment Across Shape Variation for Category-level Object Pose Refinement

Object pose refinement is essential for robust object pose estimation. Previous work has made significant progress towards instance-level object pose refinement. Yet, category-level pose refinement is a more challenging problem due to large shape variations within a category and the discrepancies between the target object and the shape prior. To address these challenges, we introduce a novel architecture for category-level object pose refinement. Our approach integrates an HS-layer and learnable affine transformations, which aims to enhance the extraction and alignment of geometric information. Additionally, we introduce a cross-cloud transformation mechanism that efficiently merges diverse data sources. Finally, we push the limits of our model by incorporating the shape prior information for translation and size error prediction. We conducted extensive experiments to demonstrate the effectiveness of the proposed framework. Through extensive quantitative experiments, we demonstrate significant improvement over the baseline method by a large margin across all metrics.

==> fig/bar_diff_initial_est/bar_diff_initial_est.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth, trim = 40 10 70 50 , clip]{fig/bar_diff_initial_est/bar_diff.pdf}
\caption{\footnotesize \textbf{diff initial est.} } 
\label{fig:bar_diff_initial_est}
\end{figure} 

==> fig/item.tex <==
\begin{figure}
% \vspace{-1mm}
\centering
\includegraphics[width=1\linewidth]{fig/placeholder.png}
\vspace{-7mm}
\caption{\footnotesize 
\textbf{Illustration of the structure.}}

\label{fig:teaser}
% \vspace{-3mm}
% \vspace{-10px}
\end{figure}             

==> fig/line_catre_vs_ours_iter/line_catre_vs_ours_5d2cm.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth, trim = 40 10 70 50 , clip]{fig/line_catre_vs_ours_iter/catre_vs_ours_5d2cm_iter.pdf}
\caption{\footnotesize \textbf{$\fiveDtwoC$ performance comparison between CATRE and our method on different initial estimations across different refining iterations.} Our methods are shown in solid lines and CATRE's are in dashed lines. Iteration 0 shows the performance of the initial estimations. {\color{blue} @Yinghan: do not forget to adjust the two graphs here}} 
\label{fig:line_iter_5d2cm}
\vspace{-10px}
\end{figure} 

==> fig/line_catre_vs_ours_iter/line_catre_vs_ours_iou75.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=1\linewidth, trim = 40 10 70 50 , clip]{fig/line_catre_vs_ours_iter/catre_vs_ours_iou75_iter.pdf}
\caption{\footnotesize \textbf{$\IoUSevenFive$ performance comparison between CATRE and our method on different initial estimations across different refining iterations.} Our methods are shown in solid lines and CATRE's are in dashed lines. Iteration 0 shows the performance of the initial estimations. {\color{blue} @Yinghan: do not forget to adjust the two graphs here}} 
\label{fig:line_iter_iou75}
\end{figure} 

==> sec/TODOs.tex <==
\section{TODOs}
{\color{blue}
TODOs:
\begin{itemize}
    \item Experiment [REAL275]: pose tracking results
    % \item Paper [Exps]: check CATRE and list necessary comparisons experiments
    % \item Paper [Exps]: think about the ablation study
    % \item Paper [Related Work]: check the point cloud feature fusion-related works
\end{itemize}}


\textbf{Subbranch ablation study:}
\begin{itemize}
    % \item Original CATRE [512 points]: done, amax, 090f7cf58d54b96f084eee13f5ed970e14d349c3
    % \item Original CATRE [use dense st branch]: done, amax, 43d1095dc3a315b4910acbfdb2cb00325588c2b6
    \item Ours [st in single branch]: {\color{blue}pending, optional}
\end{itemize}


\textbf{HSlayer pointnet encoder ablation study:}
\begin{itemize}
    % \item use HS-encoder directly: done, wangchen's machine, 
    % \item New encoder on HS-Pose: done, amax, 5a82363013b018b88438d10a3b1efb06ec77e58c
    \item hslayer in both TNet: running, shunpeng's machine
\end{itemize}

\textbf{Cross mat ablation study:}
\begin{itemize}
    \item replace cross matrix with concat: running, haoxiang's machine 
    \item no cross matrix: running, yinghan's machine
    % \item no st separate matrix (no cross mat): Done, yinghan's machine 
    \item no st separate matrix (with cross mat): {\color{blue} Pending}
    \item use transformer: {\color{blue} pending} 
    \item HSPN: parallel rts matrix: running, wangchen's machine
\end{itemize}

\textbf{Dataset Exps:}
\begin{itemize}
    \item CAMERA25: {\color{red} Needs about 30 days to train!!!,  }
    \item YCB-Video: {\color{blue}pending }
    \item YCB-Video tracking: {\color{blue}pending}
    \item LineMOD: {\color{blue}pending }
\end{itemize}

\textbf{Figures Need}
\begin{itemize}
    \item Qualitative Figures: bounding box before refinement and after, compare with CATRE (especially selecting complex shaped objects, eg mug and camera) {\color{blue}@Yinghan}
    \item Main structure figure. {\color{blue} @Wangchen}
    \item Teaser: TBD
    \item Convergence of translation and size: line graph. {\color{blue}@Yinghan, data provided by @Linfang}
\end{itemize}

\textbf{Tables Need}
\begin{itemize}
    \item Compare with SOTA
    \item Ablation Study
    \item Tracking comparison
\end{itemize}

==> tbl/ablation_for_video.tex <==
\begin{table*}
\begin{center}

% \caption{\textbf{Ablation studies on REAL275.} }
% \vspace{-4mm}
% \caption*{\footnotesize Higher score means better performance. Overall best results are in bold. Row's code in bold means the strategies taken in the final structure.}
% \label{tbl:video_ablation}
% \vspace{-3mm}
\resizebox{1\linewidth}{!}
{\footnotesize

\begin{tabular}{@{}c|l|cc|cccc|cc@{}}
\toprule

%%%% DO NOT DELETE EXPERIMENT RESULTS IN THIS TABLE. RESULTS CAN BE COMMENTED BUT NO DELETION %%%%%%%%%
Row & Method   &$\text{IoU}_{50}$    &$\text{IoU}_{75}$     &$5^\circ 2$cm &$5^\circ 5$cm &$10^\circ 2$cm &$10^\circ 5$cm &$2$cm& $5^\circ$   \\
\midrule            
\midrule            
% Method|IoU25|IoU50|IoU75|5d2cm|5d5cm|10d2cm| 10d5cm|2cm| 5deg|speed
%----------------------------
% A0 & \textbf{Ours} (full, A0 + STL + FPG + LGL)   &\textbf{84.2} &{81.9} &\underline{74.5} &\textbf{46.1} &\textbf{55.2} &\textbf{68.3} &\textbf{82.4} &\textbf{78.1} &\underline{58.3} &44/()\\ 

% \midrule
% A0 & SPD\cite{SPD_eccv_2020} (initial pose) & & & & & & & & \\
A0 & CATRE\cite{SPD_eccv_2020} (baseline)   &77.0 &43.6 &45.8 &54.4 &61.4 &73.1 &75.1 & 58.0\\
%-----------------------------------



\midrule
{B0} & A0 + prior in ST branch & {77.1} & {45.8} & {48.0} & {54.6} & {63.8} & {72.5} & {77.9} & {59.2}\\
\midrule
C0 & A0: PointNet $\rightarrow$ HS-Encoder  & 71.0 & 30.1 & 41.9 & 45.9 & 60.6 & 70.3 & 71.9 & 48.7\\
C1 & A0: PointNet $\rightarrow$ 3DGCN-Encoder &- &{28.4} & {36.0} &{43.4} &{-} &{-} &68.0 &47.7 \\ 

\midrule
{D0} & B0: PointNet $\rightarrow$ HS-layer+LATs & \textbf{79.4} & 51.0 & 52.4 & 58.6 & 69.4 & 77.7 & 80.4 & 62.4\\ 
\midrule
{E0} & \textbf{Ours}: F0+Cross-cloud Fusion&{79.2} &{\textbf{51.8}}& {\textbf{54.4}} & {\textbf{60.3}} & {\textbf{71.9}} & {\textbf{79.4}} & {\textbf{81.9}} &{\textbf{64.3}} \\
\bottomrule
\end{tabular}
}
\vspace{-10px}
\end{center}
\end{table*}

==> tbl/catre_vs_ours.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Comparison with the state-of-the-art category-level object pose refinement method (CATRE~\cite{CATRE_eccv_2022}) on REAL275 dataset.} Each comparison group contains 3 methods: the baseline pose estimation method, refinement using CATRE, and refinement using our method, respectively. {\color{red} TODO: add discription of the data reported in IoU75, which are identified with * now.}}
\label{tbl:CATRE_vs_ours}

\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{l|c|cccc}
    \toprule 
    Method &  $\text{IoU}_{75}$ & $5^\circ 2$cm & $5^\circ 5$cm & $10^\circ 2$cm & $10^\circ 5$cm \\
    \midrule
    \midrule
    DualPoseNet \cite{DualPoseNet_iccv_2021} & 30.8 & 29.3 & 35.9 & 50.0 & 66.8\\
    DualPoseNet + CATRE & 46.0 & 43.4 & 54.4 & 60.2 & 75.8\\
    DualPoseNet + Ours & 50.9 & 48.7 & 55.4 & 69.6 & 78.7 \\
    \midrule
    SelfDPDN \cite{Self-DPDN_ECCV_2022} & 42.2 & 44.3 & 50.9 & 65.1 & 78.6\\
    SelfDPDN + CATRE & 0.0 & 0.3 & 5.1 & 0.4 & 6.9 \\
    SelfDPDN + Ours & 49.7 & 53.9 & 60.1 & 75.0 & 82.8 \\
    \midrule
    GPV-Pose \cite{GPV-Pose_cvpr_2022} & 23.1* & 32.0 & 42.9 & 55.0 & 73.3\\
    GPV-Pose + CATRE & 42.6 & 39.7 & 54.1 & 57.1 & 78.0\\
    GPV-Pose + Ours & 49.6 & 47.4 & 57.8 & 68.1 & 81.2\\
    \midrule
    RBP-Pose \cite{RBP-Pose_ECCV_2022} & 24.5* & 38.2 & 48.1 & 63.1 & 79.2 \\
    RBP-Pose + CATRE & 40.0 & 41.0 & 54.7 & 60.3 & 83.7 \\
    RBP-Pose + Ours & 52.1 & 46.4 & 56.0 & 70.4 & 82.9\\
    \midrule
    HS-Pose \cite{HSPose_2023_CVPR} & 39.1* & 46.5 & 55.2 & 68.6 & 82.7\\
    HS-Pose + CATRE & 47.1 & 48.7 & 59.1 & 67.8 & 81.2 \\
    HS-Pose + Ours & 54.3 & 51.7 & 59.6 & 74.3 & 83.8\\

    \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tbl/per_cat_real275_small.tex <==
\begin{table}[ht]
\begin{center}

\caption{\textbf{Per-category results of our method on REAL275 dataset.} }
\label{tbl:per_cat_real275}
\vspace{-3mm}
\resizebox{1\linewidth}{!}
{%
\footnotesize
\begin{tabular}{@{}c|c|c|ccccc@{}}
\toprule

Method & category  & $\text{IoU}_{75}$ & $5^\circ 2\text{cm}$ & $5^\circ 5\text{cm}$ & $10^\circ 2\text{cm}$ & $10^\circ 5\text{cm}$ \\ 
\midrule
\midrule            
SPD               & bottle & 13.1 & 21.6 & 23.2 & 69.4 & 76.0 \\
SPD+\textbf{Ours} & bottle & 36.2 & 64.8 & 68.0 & 82.5 & 88.6 \\
\midrule            
SPD               & bowl   & 77.1 & 50.5 & 54.0 & 75.8 & 80.3 \\
SPD+\textbf{Ours} & bowl   & 91.9 & 91.2 & 95.6 & 95.4 & 100.0\\
\midrule            
SPD               & camera & 3.4  & 0.0  & 0.0  & 0.2  & 0.2  \\
SPD+\textbf{Ours} & camera & 12.4 & 2.1  & 2.1  & 17.9 & 18.8 \\
\midrule            
SPD               & can    & 29.8 & 37.9 & 42.7 & 80.4 & 91.6 \\
SPD+\textbf{Ours} & can    & 36.7 & 75.6 & 78.6 & 96.0 & 99.9 \\
\midrule
SPD               & laptop & 35.5 & 4.6  & 7.0  & 24.5 & 65.3 \\
SPD+\textbf{Ours} & laptop & 73.9 & 67.6 & 91.8 & 68.9 & 94.4 \\
\midrule
SPD               & mug    & 8.7  & 0.3  & 0.3  & 10.3 & 10.4 \\
SPD+\textbf{Ours} &  mug   & 59.5 & 24.8 & 25.9 & 70.7 & 74.8 \\
\bottomrule
\end{tabular}
}
\vspace{-15px}
\end{center}
\end{table}

% [1113_184537] core.catre.engine.catre_evaluator INFO@205: Inference done 2705/2754. 0.0435 s / img. ETA=0:00:02
% [1113_184539] core.catre.engine.catre_evaluator INFO@341: Total inference time: 0:02:08.386505 (0.046703 s / img per device, on 1 devices)
% [1113_184539] core.catre.engine.catre_evaluator INFO@347: Total inference pure compute time: 0:01:59 (0.043529 s / img per device, on 1 devices)
% [1113_184539] core.catre.engine.catre_evaluator INFO@356: Total inference post process time: 0:00:00 (0.000233 s / img per device, on 1 devices)
% [1113_184540] core.catre.engine.catre_custom_evaluator INFO@221: Eval recalls of results at iter=0...
% [1113_184540] core.catre.datasets.nocs INFO@290: load cached dataset dicts from /home/chenwang/Documents/Lynne/Code/My_CATRE/.cache/dataset_dicts_nocs_test_real_499b8e440e8a3c23aee21a8ce6b5ec5c.pkl
% [1113_184540] core.catre.engine.catre_custom_evaluator INFO@84: load gts of nocs_test_real
% [1113_184553] core.catre.engine.catre_custom_evaluator INFO@318: 
% objects   bottle  bowl    camera  can    laptop  mug    Avg(6)
% IoU50     49.89   99.95   43.37   69.95  82.04   66.49  68.61
% IoU75     13.09   77.13   3.38    29.77  35.48   8.69   27.92
% re5te2    21.59   50.54   0.00    37.90  4.56    0.25   19.14
% re5te5    23.18   54.00   0.00    42.69  7.04    0.25   21.19
% re10te2   69.44   75.82   0.18    80.43  24.54   10.31  43.46
% re10te5   75.95   80.30   0.20    91.59  65.31   10.39  53.96
% re10te10  87.05   80.30   0.20    91.59  65.90   10.39  55.90
% re5       35.87   54.00   0.02    45.49  7.06    0.25   23.78
% te2       80.66   94.69   34.76   87.05  29.05   85.15  68.56
% [1113_184553] core.catre.engine.catre_custom_evaluator INFO@221: Eval recalls of results at iter=1...
% [1113_184605] core.catre.engine.catre_custom_evaluator INFO@318: 
% objects   bottle  bowl    camera  can    laptop  mug    Avg(6)
% IoU25     55.99   99.95   89.54   70.54  80.36   95.13  81.92
% IoU50     50.05   99.95   64.88   70.30  78.64   86.15  75.00
% IoU75     33.92   90.76   7.54    39.27  70.15   48.35  48.33
% re5te2    55.31   88.40   0.10    70.04  62.75   17.84  49.07
% re5te5    57.60   92.85   0.10    75.26  84.92   18.74  54.91
% re10te2   85.41   95.32   3.74    92.79  64.57   55.74  66.26
% re10te5   90.81   100.00  3.98    99.84  90.76   58.89  74.05
% re10te10  100.00  100.00  4.00    99.84  95.13   58.89  76.31
% re5       79.21   93.72   0.11    78.35  89.25   18.74  59.90
% re10      100.00  100.00  4.10    99.84  96.92   58.96  76.64
% te2       85.41   95.32   53.36   92.79  64.61   87.16  79.77
% te5       90.81   100.00  97.97   99.92  91.13   99.62  96.58
% [1113_184605] core.catre.engine.catre_custom_evaluator INFO@221: Eval recalls of results at iter=2...
% [1113_184618] core.catre.engine.catre_custom_evaluator INFO@318: 
% objects   bottle  bowl    camera  can    laptop  mug    Avg(6)
% IoU25     55.11   99.95   90.05   70.54  81.29   98.04  82.50
% IoU50     50.05   99.95   75.67   70.30  80.25   92.82  78.17
% IoU75     35.40   91.04   9.12    37.56  73.19   57.13  50.58
% re5te2    61.61   88.68   1.07    72.18  71.40   24.24  53.20
% re5te5    62.75   93.29   1.07    77.24  91.25   24.72  58.39
% re10te2   83.56   95.14   12.52   93.57  72.85   67.06  70.78
% re10te5   88.68   100.00  12.97   99.88  94.43   69.72  77.61
% re10te10  100.00  100.00  13.02   99.88  96.38   69.72  79.83
% re5       85.08   93.53   1.09    79.85  92.96   24.72  62.87
% re10      100.00  100.00  13.14   99.88  96.82   69.72  79.93
% te2       83.56   95.14   54.21   93.57  72.98   89.71  81.53
% te5       88.68   100.00  98.70   99.92  95.35   99.96  97.10
% [1113_184618] core.catre.engine.catre_custom_evaluator INFO@221: Eval recalls of results at iter=3...
% [1113_184631] core.catre.engine.catre_custom_evaluator INFO@318: 
% objects   bottle  bowl    camera  can    laptop  mug    Avg(6)
% IoU25     55.11   99.95   90.05   70.54  81.69   98.87  82.70
% IoU50     50.01   99.95   77.87   70.25  80.50   95.81  79.06
% IoU75     35.44   89.86   11.56   36.46  73.60   58.81  50.95
% re5te2    64.71   89.80   3.25    74.58  69.27   24.71  54.39
% re5te5    67.21   94.10   3.25    78.51  91.86   25.57  60.08
% re10te2   82.91   95.49   17.32   94.87  70.67   69.85  71.85
% re10te5   88.80   100.00  17.85   99.96  94.64   73.67  79.15
% re10te10  100.00  100.00  17.92   99.96  95.87   73.67  81.24
% re5       88.22   94.17   3.26    80.68  92.99   25.57  64.15
% re10      100.00  100.00  18.03   99.96  96.13   73.67  81.30
% te2       82.91   95.49   57.30   94.87  70.94   90.23  81.96
% te5       88.80   100.00  98.67   99.96  95.86   99.96  97.21
% [1113_184631] core.catre.engine.catre_custom_evaluator INFO@221: Eval recalls of results at iter=4...
% [1113_184643] core.catre.engine.catre_custom_evaluator INFO@318: 
% objects   bottle  bowl    camera  can    laptop  mug    Avg(6)
% IoU50     49.77   99.95   78.40   70.25  80.75   96.20  79.22
% IoU75     36.20   91.88   12.43   36.68  73.91   59.46  51.76
% re5te2    64.77   91.17   2.13    75.64  67.61   24.83  54.36
% re5te5    68.00   95.57   2.14    78.55  91.77   25.89  60.32
% re10te2   82.50   95.44   17.94   96.01  68.92   70.73  71.92
% re10te5   88.62   100.00  18.77   99.88  94.44   74.80  79.42
% re10te10  100.00  100.00  18.89   99.88  95.62   74.80  81.53
% re5       89.10   95.65   2.15    80.69  92.50   25.89  64.33
% te2       82.50   95.44   58.26   96.01  69.34   89.86  81.90

==> tbl/pose_tracking_real275.tex <==
\begin{table*}[htbp]
\centering
\caption{\textbf{Results of category-level pose tracking on REAL275.}}
\label{tbl:pose_tracking_real275}

\begin{tabular}{l|cccccc}
    \toprule 
    Method & Oracle ICP \cite{CAPTRA_iccv_2021} & 6-PACK \cite{6D_pack_2020_ICRA} & iCaps \cite{iCaps_ral_2022} & CAPTRA \cite{CAPTRA_iccv_2021} & CATRE \cite{CATRE_eccv_2022} & Ours \\
    \midrule
    \midrule
     Init. & GT. & GT. Pert. & Det. and Seg. & GT. Pert. & GT. Pert. & \\
    \midrule
    Speed (Hz) $\uparrow$ & - & 10 & 1.84 & 12.66 & 89.21 & \\
    \midrule
    mIoU $\uparrow$ & 14.7 & - & - & 64.1 & 80.2 &\\
    $5^\circ 5$cm $\uparrow$ & 0.7 & 33.3 & 31.6 & 62.2 & 57.2 &  \\
    $\bm{R}_{\mathrm{err}}$ ($^\circ$) $\downarrow$ & 40.3 & 16.0 & 9.5 & 5.9 & 6.8 & \\
    $\bm{t}_{\mathrm{err}}$ (cm) $\downarrow$ & 7.7 & 3.5 & 2.3 & 7.9 & 1.2 & \\
    \bottomrule
\end{tabular}

\end{table*}

==> tbl/results_comparison_sota.tex <==
\begin{table*}[htbp]

\centering

\caption{\centering\textbf{Results of category-level pose refinement on REAL275 and CAMERA25 Datasets.} {\color{red} TODO: deal with the score wrt IoU75 (for SSP-Pose, others are corrected in Table 3.)}}
\label{tbl:sota_perform}

\begin{tabular}{l|l|c|c|cccc}
\toprule
Dataset & Method & Refine & $\text{IoU}_{75}$ & $5^\circ 2$cm & $5^\circ 5$cm & $10^\circ 2$cm & $10^\circ 5$cm  \\ 

\midrule
\midrule

\multirow{14}{*}{REAL275} 
    & NOCS \cite{NOCS_cvpr_2019}  &  & 9.4 & 7.2 & 10.0 & 13.8 & 25.2 \\
    & DualPoseNet \cite{DualPoseNet_iccv_2021} & \checkmark & 30.8 & 29.3 & 35.9 & 50.0 & 66.8 \\
    & CR-Net \cite{CR-Net_iros_2021} &  & 33.2 & 27.8 & 34.3 & 47.2 & 60.8 \\
    & SGPA \cite{SGPA_iccv_2021} &  & 37.1 & 35.9 & 39.6 & 61.3 & 70.7 \\
    & SAR-Net \cite{SAR-Net_Lin_2022_CVPR} & & - & 31.6 & 42.3 & 50.3 & 68.3 \\
    & SSP-Pose \cite{SSP-Pose_IROS_22} & & - & 34.7 & 44.6 & - & 77.8 \\
    & RBP-Pose \cite{RBP-Pose_ECCV_2022} & & 67.8× & 38.2 & 48.1 & 63.1 & 79.2 \\
    & GPV-Pose \cite{GPV-Pose_cvpr_2022} & & 64.4× & 32.0 & 42.9 & 55.0 & 73.3 \\
    & SPD$^*$ \cite{SPD_eccv_2020} &  & 27.0 & 19.1 & 21.2 & 43.5 & 54.0 \\ 
    & HS-Pose \cite{HSPose_2023_CVPR} & & 74.7× & 46.5 & 55.2 & 68.6 & 82.7\\ \cline{2-8}
    & SPD$^*$$+$CATRE \cite{CATRE_eccv_2022} & \checkmark & 43.6 & 45.8 & 54.4 & 61.4 & 73.1 \\
    & SPD$^*$$+$Ours & \checkmark & 51.8 & 54.4 & 60.3 & 71.9 & 79.4 \\ 
    & HS-Pose + CATRE & \checkmark & 47.1 & 48.7 & 59.2 & 67.8 & 81.2 \\
    & HS-Pose + Ours & \checkmark & 55.4 & 52.5 & 59.0 & 74.4 & 82.3 \\
\midrule

\multirow{14}{*}{CAMERA25} 
    & NOCS \cite{NOCS_cvpr_2019}  &  & 37.0 & 32.3 & 40.9 & 48.2 & 64.6 \\
    & DualPoseNet \cite{DualPoseNet_iccv_2021} & \checkmark & 71.7 & 64.7 & 70.7 & 77.2 & 84.7 \\
    & CR-Net \cite{CR-Net_iros_2021} &  & 75.0 & 72.0 & 76.4 & 81.0 & 87.7 \\
    & SGPA \cite{SGPA_iccv_2021} &  & 69.1 & 70.7 & 74.5 & 82.7 & 88.4 \\
    & SAR-Net \cite{SAR-Net_Lin_2022_CVPR}& & - & 66.7 & 70.9 & 75.3 & 80.3 \\
    & SSP-Pose \cite{SSP-Pose_IROS_22}& & - & 64.7 & 75.5 & - & 87.4 \\
    & RBP-Pose \cite{RBP-Pose_ECCV_2022}& & - & 73.5 & 79.6 & 82.1 & 89.5\\
    & GPV-Pose \cite{GPV-Pose_cvpr_2022}& & - & 72.1 & 79.1 & - & 89.0\\
    & HS-Pose \cite{HSPose_2023_CVPR} & & - & 73.3 & 80.5 & 80.4 & 89.4\\ 
    & SPD$^*$ \cite{SPD_eccv_2020} &  & 46.9 & 54.1 & 58.8 & 73.9 & 82.1 \\ 
    \cline{2-8}
    & SPD$^*$$+$CATRE \cite{CATRE_eccv_2022} & \checkmark & 76.1 & 75.4 & 80.3 & 83.3 & 89.3 \\
    & SPD$^*$$+$Ours & \checkmark & {79.2} & {77.9} &{84.0} &{83.8} &{90.5} \\
    & HS-Pose + CATRE & \checkmark & & & & &\\
    & HS-Pose + Ours & \checkmark & & & & &\\
\bottomrule
\end{tabular}

\end{table*}
